Effective Edge Centrality via Neighborhood-based Optimization

Given a network G, edge centrality is a metric used to evaluate the importance of edges in G, which is a key concept in analyzing networks and finds vast applications involving edge ranking. In spite of a wealth of research on devising edge centrality measures, they incur either prohibitively high computation costs or varied deficiencies that lead to sub-optimal ranking quality. To overcome their limitations, this paper proposes ECHO, a new centrality measure for edge ranking that is formulated based on neighborhood-based optimization objectives. We provide in-depth theoretical analyses to unveil the mathematical definitions and intuitive interpretations of the proposed ECHO measure from diverse aspects. Based thereon, we present three linear-complexity algorithms for ECHO estimation with non-trivial theoretical accuracy guarantees for centrality values. Extensive experiments comparing ECHO against six existing edge centrality metrics in graph analytics tasks on real networks showcase that ECHO offers superior practical effectiveness while offering high computation efficiency.

==> solution.tex <==
\section{Methodology}

\cite{kucharczuk2022pagerank}

\begin{lemma}
Let $\EM \in \mathbb{R}^{m\times n}$ be the incidence matrix of $G$, where $\EM[e_{i,j},v_i]=1$ and $\EM[e_{i,j},v_j]=-1$ for each edge $e_{i,j}\in E$  with two end points $v_i,v_j$, $\EM[e_{i,j},v_x]=0$ if $v_x\neq v_i,v_j$. We have $\LM=\EM^{\top}\EM$.
\begin{proof}
Recall that $\LM =\DM-\AM$. Thus, for any node $v_i\in V$, $\LM_{i,i}=d(v_i)$ and for any edge $(v_i,v_j)\in E$, $\LM_{i,j}=\LM_{j,i}=-1$. For any two nodes $v_i,v_j$ such that $v_i\neq v_j$ and $(v_i,v_j)\notin E$, $\LM_{i,j}=\LM_{j,i}=0$.

for any two nodes $v_i,v_j\in V$, $\EM[v_i]\cdot \EM[v_j]=\sum_{e\in E}{\EM[e,v_i]\cdot \EM[e,v_j]}$. 
By definition, if $v_i=v_j$, we have $\EM[v_i]\cdot \EM[v_j]= d(v_i)$.
Note that if node $v_i$ (resp. $v_j$) is not incident to $e$, $\EM[v_i,e]=0$ (resp. $\EM[v_j,e]=0$). So, if $(v_i,v_j)\notin E$ and $(v_j,v_i)\notin E$, we have $\EM[v_i]\cdot \EM[v_j]=0$. If $(v_i,v_j) \in E$ or $(v_j,v_i) \in E$, $\EM[v_i]\cdot \EM[v_j]=\EM[e_{i,j},v_i]\cdot \EM[e_{i,j},v_j]+\EM[e_{j,i},v_j]\cdot \EM[e_{j,i},v_i]=-1$. Therefore, the lemma is proved.
\end{proof}
\end{lemma}


We define matrix $\QM\in \mathbb{R}^{m\times m}$
\begin{equation}\label{eq:Q}
\QM 
% = \EM\cdot \sum_{\ell=0}^{\infty}{\PM^{\ell}} \DM^{-1}\cdot \EM^{\top} 
=\EM\LM^{+}\EM^{\top}
\end{equation}

\begin{theorem}
$r(e_{i,j})=\QM[e_{i,j}, e_{i,j}]$ holds for every edge $e_{i,j}\in E$.
\begin{proof}
We first prove $\QM[e_{i,j},e_{i,j}]=r(e_{i,j})$ holds for every edge $e_{i,j}\in E$.

$(\EM\LM^{+})[e_{i,j},v_x]=\EM[e_{i,j}]\cdot \LM^{+}[:,v_x]=\LM^{+}[v_i,v_x]-\LM^{+}[v_j,v_x]$. 

This means $(\EM\LM^{+})[e_{i,j},v_i]=\LM^{+}[v_i,v_i]-\LM^{+}[v_j,v_i]$ and $(\EM\LM^{+})[e_{i,j},v_j]=\LM^{+}[v_i,v_j]-\LM^{+}[v_j,v_j]$.

So $(\EM\LM^{+})[e_{i,j},v_i]-(\EM\LM^{+})[e_{i,j},v_j]=r(e_{i,j})$.
Then $\QM[e_{i,j},e_{i,j}]=(\EM\LM^{+}\EM^{\top})[e_{i,j},e_{i,j}]=(\EM\LM^{+})[e_{i,j},v_i]-(\EM\LM^{+})[e_{i,j},v_j]=r(e_{i,j})$.

% First, $\EM^{\top}\EM=\LM=\DM-\AM$.
% % According to \cite{peng2021local,andoni2019solving}, 
% $\LM=\DM-\AM$. Since $\LM^{+}$ is the Moore-Penrose Pseudoinverse of $\LM$, then $\LM^{+}\LM\LM^{+}=\LM^{+}$. Also, easy to prove see $\QM$ is symmetric.
% \begin{align*}
% \QM&=\EM\LM^{+}\EM^{\top}=\EM\LM^{+}\LM\LM^{+}\EM^{\top}=\EM\LM^{+}(\DM-\AM)\LM^{+}\EM^{\top}=\EM\LM^{+}\EM^{\top}\EM\LM^{+}\EM^{\top}=\QM\QM^{\top}.
% \end{align*}
% This means $r(e_{i,j})=\QM[e_{i,j},e_{i,j}]=\QM[e_{i,j}]\cdot \QM[e_{i,j}]=\|\QM[e_{i,j}]\|^2_2$.
The theorem is proved.
\end{proof}
\end{theorem}

By Section 2.2 in \cite{spielman2008graph},
\begin{equation}
\LM=\UM\boldsymbol{\Lambda}\UM^{\top}, \LM^{+}=\UM \boldsymbol{\Lambda}^{-1}\UM^{\top}.
\end{equation}

Let $\UM\boldsymbol{\Sigma}\VM^{\top}$ be the SVD of $\EM^{\top}$. Note that $\UM$ and $\VM$ are semi-unitary matrices, i.e., $\UM^{\top}\UM=\VM^{\top}\VM=\IM$. An interesting observation is that
$\LM=\EM^{\top}\EM = \UM\boldsymbol{\Sigma}\VM^{\top}\VM\boldsymbol{\Sigma}\UM^{\top}=\UM\boldsymbol{\Sigma}^2\UM^{\top}$. So, $\LM^{+}=\UM\frac{1}{\boldsymbol{\Sigma}^2}\UM^{\top}$. So, $\QM=\EM\LM^{+}\EM^{\top}=\VM\boldsymbol{\Sigma}\UM^{\top}\cdot\UM\frac{1}{\boldsymbol{\Sigma}^2}\UM^{\top}\cdot \UM\boldsymbol{\Sigma}\VM^{\top}=\VM\VM^{\top}$.


% https://www.cs.utexas.edu/~ecprice/courses/randomized/fa21/scribe/lec17.pdf
Let $\SM \in \mathbb{R}^{m \times m}$ be a diagonal matrix, where each element satisfy
\begin{equation}
\SM[e_{i,j},e_{i,j}] = \frac{\text{\# of times edge}\ e_{i,j}\ \text{is sampled}}{n_s}\cdot \frac{r(e_{i,j})}{n-1}
\end{equation}
We have
\begin{equation}
\LM^{\prime} = \EM\SM\EM^{\top},
\end{equation}
which is a sparsified version of the graph Laplacian $\LM$.
